Adversarial Genetic Programming for Cyber Security: A Rising Application Domain Where GP Matters

Cyber security adversaries and engagements are ubiquitous and ceaseless. We delineate Adversarial Genetic Programming for Cyber Security, a research topic that, by means of genetic programming (GP), replicates and studies the behavior of cyber adversaries and the dynamics of their engagements. Adversarial Genetic Programming for Cyber Security encompasses extant and immediate research efforts in a vital problem domain, arguably occupying a position at the frontier where GP matters. Additionally, it prompts research questions around evolving complex behavior by expressing different abstractions with GP and opportunities to reconnect to the Machine Learning, Artificial Life, Agent-Based Modeling and Cyber Security communities. We present a framework called RIVALS which supports the study of network security arms races. Its goal is to elucidate the dynamics of cyber networks under attack by computationally modeling and simulating them.

==> challenges.tex <==
The past work reviewed in the previous section indicates that, first,
there are opportunities that can be approached by combining
adversarial evolution and GP (~\ref{sec:opport-gp-advers}), and
second, there are also several challenges
(~\ref{sec:challenges}). This section highlights these.

\subsection{Opportunities for GP and Adversarial Evolution}
\label{sec:opport-gp-advers}

We have identified the following opportunities:
\begin{asparadesc}
\item [Adversarial Evolution] When dealing with intelligent
  adversaries as in security and tax
  evasion~\cite{hemberg2015icail,alec18}, the adversaries innovate to
  nullify the solutions provided to contain them. An EA ignores the
  coupling of the adversaries and it only evolves one. Thus the final
  solutions is fragile, i.e. not robust to the inevitable change of
  the adversaries' posture(\tests).  Therefore, there exists a need of
  mimicking the arms-race in which both adversaries evolve, ergo
  \CompCA.
\item [Executable Variable Length Representation] Many studies address
  cybersecurity problems by providing solutions defined by fixed set
  of configuration parameters to define a defense
  strategy~\cite{ostaszewski2007coevolutionary,rush2015coevolutionary}.
  These cyberdefenses are often executable structures, with behavior
  determined by the configuration parameters.  The simply modifying
  the parameters limits the exploration of new strategies. Another
  concern is the non-trivial task of determining the appropriate size
  for complex problems~\cite{stanley2004competitive}.

  GP has the ability to evolve variable length formal executable
  structures (e.g. programs, protocols or state machines) over a
  ``theoretically infinite'' search space.  In combination with the
  use of adversarial evolution, \CompCA GP provides a framework to
  compute robust potentially novel defense solutions.

\item [Open-ended coevolution] GP facilitate the definition of
  open-end arms-race since it presents the essential ingredients of
  open-ended evolution, which are: a dynamically changing fitness
  landscape, availability of adversarial process, and search with
  continuously injected randomness~\cite{ONeill2010}.

\end{asparadesc}

\subsection{Challenges}
\label{sec:challenges}

Applying adversarial GP to address security problems offers a
promising research opportunities.  However, there are several
challenges. In this section, we discuss the most prominent.

\begin{asparadesc}
\item [Subjective Solution Evaluation] \CAs compare the individuals on
  basis of their interaction with other individuals, and therefore,
  the evaluation of individuals is subjected to the changing
  adversaries and can only provide relative ordering. For this reason,
  the fitness in \CAs is called \textit{subjective fitness}.  This
  change over traditional EAs generates a variety fundamental
  differences~\cite{popovici2012coevolutionary,popovici2015framework}.

\item [Algorithm operator and parameter selection] What GP and \CompCA
  model should be used, this is a common modelling problem, but the
  \CompCA provides additional model and parameter selection choices,
  e.g. which solution concept to use. In addition, GP has its own set
  of challenges~\cite{ONeill2010}, e.g. bloat, which search
  operators.

\item[Evaluation Computational Cost] The individual's fitness is
  evaluated based on its interaction with other individuals.  A
  concern for \CompCAs is the number of fitness evaluations. Thus,
  many \CompCAs methods try to reduce fitness evaluations,
  e.g. \cite{kimclustering,liskowski2016non,mitchell2006coevolutionary,liskowski2017online,bari2018selection}.
 
\item[Solution Validation] Modeling and simulation comprise a powerful
  approach for mimicking actual conditions, and lack of
  data~\cite{popovici2017bridging}.  Using such tools one can evaluate
  the solutions in a number of security scenarios, computer security,
  and network dynamics. However, it is important to chose the proper
  simulator, since it limits important aspects of the work as the
  level of abstraction of the solution to be applied (i.e., the
  problem to be addressed) or the realism of the provided results. The
  challenge is to validate solutions that have been proposed.

\end{asparadesc}

This section highlighted the opportunities and challenges for
adversarial GP. The next section intorduces the \RIVALS framework, an
attempt to provide GP that matters, here in the domain of network
security.



==> conclusions.tex <==
\section{Conclusions}

